Limits and consistency of non-local and graph approximations to the Eikonal equation

In this paper, we study a non-local approximation of the time-dependent (local) Eikonal equation with Dirichlet-type boundary conditions, where the kernel in the non-local problem is properly scaled. Based on the theory of viscosity solutions, we prove existence and uniqueness of the viscosity solutions of both the local and non-local problems, as well as regularity properties of these solutions in time and space. We then derive error bounds between the solution to the non-local problem and that of the local one, both in continuous-time and Backward Euler time discretization. We then turn to studying continuum limits of non-local problems defined on random weighted graphs with $n$ vertices. In particular, we establish that if the kernel scale parameter decreases at an appropriate rate as $n$ grows, then almost surely, the solution of the problem on graphs converges uniformly to the viscosity solution of the local problem as the time step vanishes and the number vertices $n$ grows large.

==> sections/sec_existence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Existence}






==> sections/sec_mainresults_backward.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Backward Euler discrete time non-local to local error bound}\label{subsec:eikconvdiscrete}
We consider the time-discrete approximation of \eqref{cauchy-J} using backward Euler discretization. Then we will show an error estimate between a solution of this equation with the continuous viscosity solution of \eqref{cauchy}.

Using the backward/implicit Euler discretization scheme, a time-discrete counterpart of \eqref{cauchy-J} reads
\begin{equation}\tag{\textrm{$\mathcal{P}_{\e}^{\rm{BD}}$}}\label{cauchy-J-discrete-bw}
\begin{cases}
\frac{f^\e(u,t) - f^\e(u,t-\Delta t)}{\Delta t} = - \abs{ \nabla_{J_\e}^- f^\e(u,t)}_\infty + \tilde{P}(u),  & (u,t) \in   (\tilde{\Omega} \setminus \tilde{\Gamma}) \times \set{t_1,\ldots,t_{N_T}} ,\\
f^\e(u,t) = \tilde{\psi} (u), & (u,t) \in \partial\tilde{\Omega}_{N_T} ,
\end{cases}
\end{equation}
where $t_{i} = i \Delta t$ for all $i \in \set{0,\ldots,N_T}$. 

In Appendix~\ref{sec:cauchy-J-discrete}, we prove that \eqref{cauchy-J-discrete-bw} is well-posed. Indeed, Lemma~\ref{discrete-existence} shows existence of a discrete-time solution (in the sense of Definition~\ref{def:discretesolution}). Our method of proof is constructive giving a practical way to build such a solution. Uniqueness follows from the comparison principle in Lemma~\ref{lem-comparison}.

\tcb{
\begin{rem}
Computing numerically the solution \eqref{cauchy-J-discrete-bw} amounts to computing the resolvent of $\abs{\nabla_{J_\e}^- \cdot}_\infty$ subject to the boundary constraint. Though we will not elaborate more on this since the paper is essentially theoretial, this problem could be solved using primal-dual proximal splitting algorithms \cite{chambolle2011first}. We leave this to a future work.
\end{rem}
}

We are now in position to state the following error estimate.
\tcb{
\begin{thm}\label{thm:discrete-bw-estimate}
Let $T>0$ and $\e \in ]0,1]$. Suppose that assumptions~\ref{assum:Om}--\ref{assum:compatdomains} hold, and that  $\distH(\Gamma,\tilde \Gamma) = O(\e^{\min(\nu,1/2)})$. Let $f$ be the unique viscosity solution of \eqref{cauchy} and $f^\e$ be a solution of \eqref{cauchy-J-discrete-bw}. Then there exists a constant $K > 0$ depending only on the dimension $m$, $\norm{\psi}_{L^\infty(\Omega)}$, $\norm{P}_{L^\infty(\Omega\setminus\Gamma)}$, $\Lip{\psi}$, $\Lip{\tilde{\psi}}$, $\Lip{P}$, $\Lip{\tilde{P}}$ and $c_g$ such that for any $\e$ small enough
\begin{align*}
\normL{f^\e-f}_{L^\infty\pa{\tilde{\Omega} \times \set{0,\ldots,t_{N_T}}}}  
\leq K(T+1)(\e^{\min(\nu,1/2)} + \Delta t^{1/2})
+ T\normL{P - \tilde{P}}_{L^\infty(\tilde{\Omega}\setminus\tilde{\Gamma})} 
+ \normL{\psi - \tilde{\psi}}_{L^\infty(\tilde{\Omega})} .
\end{align*}
In particular, if $\tilde{P}=P$ on $\tilde{\Omega}\setminus\tilde{\Gamma}$ and $\tilde{\psi}=\psi$ on $\tilde{\Omega}$, then 
\begin{align*}
\lim_{\e \to 0, \Delta t \to 0} \normL{f^\e-f}_{L^\infty\pa{\tilde{\Omega} \times \set{0,\ldots,t_{N_T}}}}  = 0 .
\end{align*}
\end{thm}
}

The proof is quite similar to the one of Theorem~\ref{thm:continuous-time-estimate}. We highlight only the steps where we have to handle properly the discrete time approximation. For instance, we will need the Lipschitz regularity properties of $f^\e$ both in time and space (see Lemma~\ref{lem-lip-bw}).

\begin{proof}
Again, $K$ will denote in this proof any positive constant that depends only on the data, but may change from one line to another. Here we focus on the case $f-f^\e$ on purpose to complement the details provided in the proof Theorem~\ref{thm:continuous-time-estimate}. 

\begin{enumerate}[label=Step~\arabic*.]
\item {\em Test-function and maximum point.} 

For $\gamma > 0$ and $\eta > 0$, we consider maximizing over $\Omega_T \times \tilde{\Omega}_{N_T}$ the test-function
\begin{eqnarray*}\label{varphi}
\Psi_{\gamma,\eta}(x,t,u,s)= f(x,t) - f^\e(u,s) - \frac{|x-u|^2}{2\gamma} -\frac{|t-s|^2}{2\gamma} - \eta t.
\end{eqnarray*}

Since $\Omega_T \times \tilde{\Omega}_{N_T}$ is compact and $\Psi_{\gamma,\eta}$ is continuous, the maximum is attained at some point $(\bar{x},\bar{t}, \bar{u},\bar{t}_i)$. Exactly as in the proof of Theorem~\ref{thm:continuous-time-estimate}, we have
%
\begin{align}
|\bar{x}-\bar{u}| &\leq K \gamma \label{lip-pro-x} \qandq \\
|\bar{t} - \bar{t}_i| &\leq (K+\eta) \gamma. \label{lip-pro-t}
\end{align}


\item {\em Excluding interior points from the maximum.}

\noindent We show that for $\eta$ large enough, we have either $(\bar{x},\bar{t}) \in \partial \Omega_T$ or $(\bar{u},\bar{t}_i) \in \partial \tilde{\Omega}_{N_T}$. We argue again by contradiction and assume that $(\bar{x},\bar{t}) \in  \Omega\setminus \Gamma \times ]0,T[$  and $(\bar{u},\bar{t}_i) \in   \tilde{\Omega}\setminus \tilde \Gamma \times \{t_1,\dots, t_{N_T}\}$. Using that $(\bar{x},\bar{t})$ is a maximum point of the function $(x,t) \mapsto \Psi_{\gamma,\eta}(x,t, \bar{u},\bar{t}_i) $ and the fact that $f$ is a  viscosity sub-solution of \eqref{cauchy}, we have
%
\begin{eqnarray}\label{1st-ineq}
\eta + \frac{\bar{t} - \bar{t}_i}{\gamma} \leq - \frac{|\bar{x}-\bar{u}|}{\gamma} + P(\bar{x}).
\end{eqnarray}

Using now that $\bar{t}_i > 0$ and that $f^\e$ is a solution of \eqref{cauchy-J-discrete-bw}, we have
\begin{equation}\label{2nd-ineq}
\frac{f^\e(\bar{u},\bar{t}_i) - f^\e(\bar{u},\bar{t}_i-\Delta t)}{\Delta t} = - \babs{\nabla_{J_\e}^- f^\e(\bar{u},\bar{t}_i)}_\infty + \tilde{P}(\bar{u}).
\end{equation}
%
We set $\varphi: (u,s) \in \tilde{\Omega}_{N_T} \mapsto f(\bar x,\bar t) - \frac{|\bar{x}-u|^2}{2\gamma} -\frac{|\bar{t}-s|^2}{2\gamma} - \eta \bar{t}$. In particular, $(\bar{u},\bar{t}_i)$ is the minimum point of $f^\e-\varphi$ over $\tilde{\Omega}_{N_T}$. This implies that
%
\begin{eqnarray*}
f^\e(\bar{u},\bar{t}_i) - f^\e(\bar{u},\bar{t}_i- \Delta t) \leq \varphi (\bar{u},\bar{t}_i) -\varphi(\bar{u},\bar{t}_i - \Delta t),
\end{eqnarray*}
%
and so
\begin{eqnarray}\label{ineq-1}
\frac{f^\e(\bar{u},\bar{t}_i) - f^\e(\bar{u},\bar{t}_i- \Delta t) }{\Delta t} \leq \frac{\bar{t} - \bar{t}_i}{\gamma} + \frac{\Delta t}{2 \gamma}.
\end{eqnarray}
%
$(\bar{x},\bar{t},\bar{u},\bar{t}_i)$ is a maximizer of $\Psi_{\gamma,\eta}$, whence we get 
\[
f^\e(\bar{u},\bar{t}_i) - f^\e(v,\bar{t}_i) \leq \frac {|\bar{x} - v|^2 - |\bar{x} - \bar{u}|^2}{2\g}, \qquad \forall v \in \tilde{\Omega} .
\]
Thus we estimate the right hand side of \eqref{2nd-ineq} to show that
\begin{equation}\label{ineq-2}
\begin{aligned}
\babs{\nabla_{J_\e}^- f^\e(\bar{u},\bar{t}_i)}_\infty
&=  \max_{v\in\tilde{\Omega},|\bar{u}-v| \in \e\Sg}J_\e(\bar{u},v) (f^\e(\bar{u},\bar{t}_i) -f^\e(v,\bar{t}_i)) \\
&\leq (2\gamma)^{-1}\max_{v\in\tilde{\Omega},|\bar{u}-v| \in \e\Sg} J_\e(\bar{u},v)\pa{|\bar{x}-v|^2 - |\bar{x}-\bar{u}|^2} \\
&=  (2\gamma)^{-1}\max_{v\in\tilde{\Omega},|\bar{u}-v| \in \e\Sg} J_\e(\bar{u},v)\bpa{|\bar{x}-v| - |\bar{x}-\bar{u}|}\bpa{|\bar{x}-v| - |\bar{x}-\bar{u}| + 2 |\bar{x}-\bar{u}|}  \\
&\le (2\gamma)^{-1}\max_{v\in\tilde{\Omega},|\bar{u}-v| \in \e\Sg} J_\e(\bar{u},v){|\bar{u}-v|}\bpa{|\bar{u}-v| + 2 |\bar{x}-\bar{u}|}  \\
&\leq  \max_{v\in\tilde{\Omega},|\bar{u}-v| \in \e\Sg} \frac{|\bar{x}-\bar{u}|}{\gamma} \frac{|\bar{u}-v|}{C_g \e} g\pa{\frac{|\bar{u}-v|}{\e}} \\
&+ \max_{v\in\tilde{\Omega},|\bar{u}-v| \in \e\Sg} \frac{|\bar{u}-v|^2}{2\gamma C_g \e} g\pa{\frac{|\bar{u}-v|}{\e}} \\
&\leq  \frac{|\bar{x}-\bar{u}|}{\gamma} + r_g\frac{\e}{2\gamma} .
%\leq  \frac{|\bar{x}-\bar{u}|}{\gamma} + K\frac{\e}{\gamma} .
\end{aligned}
\end{equation}
%\end{equation}
%\begin{equation}\label{ineq-2}
%\babs{\nabla_{J_\e}^- f^\e(\bar{u},\bar{t}_i)}_\infty
%\leq  \frac{|\bar{x}-\bar{u}|}{\gamma} + K\frac{\e}{\gamma} .
%\end{equation}

Plugging \eqref{ineq-1} and \eqref{ineq-2} into \eqref{2nd-ineq} we get
%
\begin{eqnarray}\label{3rd-ineq}
\frac{\bar{t} - \bar{t}_i}{\gamma} + \frac{\Delta t}{2 \gamma} \geq  -  \frac{|\bar{x}-\bar{u}|}{\gamma} - K\frac{\e}{\gamma} + \tilde{P}(\bar{u}).
\end{eqnarray}
%
From \eqref{1st-ineq} and \eqref{3rd-ineq}, we finally obtain
%
\begin{eqnarray*}
\eta &\leq& K\frac{\Delta t + \e}{\gamma} + P(\bar{x}) - \tilde{P}(\bar{u})\\
&\leq&  K\frac{\Delta t + \e}{\gamma} + K |\bar{x}-\bar{u}| + \normL{P - \tilde{P}}_{L^\infty(\tilde{\Omega} \setminus \tilde{\Gamma})} \\
&<& K \pa{\frac{\Delta t + \e}{ \gamma}  + \gamma}+\normL{P - \tilde{P}}_{L^\infty(\tilde{\Omega} \setminus \tilde{\Gamma})} \eqdef \bar{\eta}.
\end{eqnarray*}
We then conclude that either $(\bar{x},\bar{t}) \in \partial \Omega_T$ or $(\bar{u},\bar{t}_i) \in \partial \tilde{\Omega}_{N_T}$ for $\eta\ge \bar \eta$. \tcb{When reverting the roles of $f^\e$ and $f$, only $\bar{\eta}$ will be changed taking an additional term $\e^\nu$ (see the proof of Theorem~\ref{thm:continuous-time-estimate})}. The rest of the proof is exactly the same as \ref{step:proofconclusion} in the proof of Theorem~\ref{subsec:eikconvcont}, where we now invoke Lemma~\ref{lem-lip-bw}.
%\JF{The rest of the proof is exactly the same as \ref{step:proofconclusion} in the proof of Theorem~\ref{subsec:eikconvcont}.} \todo{This is not true. The case $\bar{t}=0$ is rather easy to take care of by using the Lipschitz regularity in time of the scheme given by Lemma~\ref{lem-lip-bw}. However, the case $\bar{x} \in \Gamma$ does not work since we invoke \ref{assum:psisssol-J} and \eqref{eq:barrier-f-J} with the barrier $\tilde{\psi}_b$. We thus need an adaptation of these notions/results to the time-discrete setting.}
\end{enumerate}
\end{proof}

